Neural Network Verification for Gliding Drone Control: A Case Study

As machine learning is increasingly deployed in autonomous systems, verification of neural network controllers is becoming an active research domain. Existing tools and annual verification competitions suggest that soon this technology will become effective for real-world applications. Our application comes from the emerging field of microflyers that are passively transported by the wind, which may have various uses in weather or pollution monitoring. Specifically, we investigate centimetre-scale bio-inspired gliding drones that resemble Alsomitra macrocarpa diaspores. In this paper, we propose a new case study on verifying Alsomitra-inspired drones with neural network controllers, with the aim of adhering closely to a target trajectory. We show that our system differs substantially from existing VNN and ARCH competition benchmarks, and show that a combination of tools holds promise for verifying such systems in the future, if certain shortcomings can be overcome. We propose a novel method for robust training of regression networks, and investigate formalisations of this case study in Vehicle and CORA. Our verification results suggest that the investigated training methods do improve performance and robustness of neural network controllers in this application, but are limited in scope and usefulness. This is due to systematic limitations of both Vehicle and CORA, and the complexity of our system reducing the scale of reachability, which we investigate in detail. If these limitations can be overcome, it will enable engineers to develop safe and robust technologies that improve people's lives and reduce our impact on the environment.

==> intro-argument.tex <==
1. Verification of NN controllers is a fast growing field.

What goes in this para: when this research started, what tools involves, ARCH competition, what sort of famous/popular benchmarks it uses

2. Some standard verification "pipelines"/methods have been developed by this community, that involve property-guided training and verification. 

Explain why integration of these two is important, who pioneered these methods, what major publications/applications exist. Thomas'es work, Marco's work etc.
Maybe a picture of pipeline will help (or cycle between NNV and training)

3. Bioinspired gliding drones have not yet received any attention by that community, but they present a promising case for verification. 

What goes in this para: what these drones are, how popular, what they are used for, why NN as controllers, why it is important to verify them -- pretty much the text you currently have, maybe you will sharpen it a bit, so that it fits better with the main story line...

4. At the same time, they present a challenge for neural network verification.

This is a very important para, that needs to explain how NN controllers used in bioinspired gliding drones present different verification challenges compared to standard ARCH benchmarks. How/why property-guided training that was developed for classification tasks does not work here

5. Solving these challenges will require introduction of several modifications to the standard neural network verification pipeline. 

Explain what modifications you propose are needed, and why they are needed.

6. In this paper we present a case study that substantiates this claim, using two examples of  Bioinspired gliding drones / an example of Alsomitra

Here: explain major highlights and conclusions of the study. 
